The telescope conjecture at height 2 and the tmf resolution

Mahowald proved the height 1 telescope conjecture at the prime 2 as an application of his seminal work on bo-resolutions. In this paper we study the height 2 telescope conjecture at the prime 2 through the lens of tmf-resolutions. To this end we compute the structure of the tmf-resolution for a specifc type 2 complex Z. We find that, analogous to the height 1 case, the E1-page of the tmf-resolution possesses a decomposition into a v2-periodic summand, and an Eilenberg-MacLane summand which consists of bounded v2-torsion. However, unlike the height 1 case, the E2-page of the tmf-resolution exhibits unbounded v2-torsion. We compare this to the work of Mahowald-Ravenel-Shick, and discuss how the validity of the telescope conjecture is connected to the fate of this unbounded v2-torsion: either the unbounded v2-torsion kills itself off in the spectral sequence, and the telescope conjecture is true, or it persists to form v2-parabolas and the telescope conjecture is false. We also study how to use the tmf-resolution to effectively give low dimensional computations of the homotopy groups of Z. These computations allow us to prove a conjecture of the second author and Egger: the E(2)-local Adams-Novikov spectral sequence for Z collapses.

==> table.tex <==
% !TEX root = tmfASSZ2.tex



\begin{center}
\begin{tabular}{|  c | c | c | }
\hline
Name & Description & Location \\
\hline
\hline
$\Sigma(2) $ &   $ \mathbb{F}_{2}[v_2^{\pm1}][t_1, t_2, \ldots]/(t_k^{4} - v_2^{2^k-1}t_k)$  &   \eqref{eq:Sidef} \\
$\Sigma_2$  &  $ \mathbb{F}_{4}[u^{\pm1}][ t_1, t_2, \ldots]/(t_k^{4} - v_2^{2^k-1}t_k)$ &   \eqref{eq:Siexdef}  \\
$\overline{\Sigma}_2 $ & $ \FF_4[u^{\pm 1}][\tb_2, \tb_3, \cdots ]/ (\tb_2^2 - \omega v_2 \tb_2, \tb_k^4 - v_2^{2^k-1}\tb_k)$ & \eqref{eq:barSigma_2} \& \eqref{eq:sidef}  \\
$ \br{\Sigma}(2)$ &   $\br{\Sigma}_2^{C_3} \cong \FF_4[v_2^{\pm1}][\tb_2, \tb_3, \cdots ]/ (\tb_2^2 - \omega v_2 \tb_2, \tb_k^4 - v_2^{2^k-1}\tb_k)$ & Cor.~\ref{cor:brSidesc}   \\
$\td{\Sigma}(2)$ & $\br{\Sigma}(2)^{\Gal}$ & Sec.~\ref{sec:subhopf}  \\
$\si(2)$ &  $\FF_2[v_2] [t_1, t_2, \ldots]/(t_k^{4}-v_2^{2^k-1}t_k)$ &  \eqref{eq:sidef} \\
$\sibr(2)$   & $ \FF_4[v_2][\td{t^2_2}, \tb_3, \cdots ]/ ((\td{t_2^2})^2 + v_2^2 \td{t^2_2}, \tb_k^4 + v_2^{2^k-1}\tb_k)$ & \eqref{eq:sibrdef}  \\
$\sitd(2)$  & $\FF_2[v_2^{\pm1}][\td{t^2_2}, \td{t}_3, \ldots ]/((\td{t_2^2})^2 = v^2_2 \td{t_2^2}, \: \td{t}_k^4 = \text{terms AF $> 0$}) $ & Def.~\ref{defn:S2tilde} \& Th.~\ref{thm:goodcomplex}\\
\hline
\end{tabular}
\end{center}


\begin{figure}
\begin{center}
\begin{tabular}{|  c | c | }
\hline
Name & Location  \\
\hline
\hline
$\Sigma(2) $   &   \eqref{eq:Sidef} \\
$\Sigma_2$  &   \eqref{eq:Siexdef}  \\
$\overline{\Sigma}_2 $ & \eqref{eq:barSigma_2} \& \eqref{eq:defbrSiext}  \\
$ \br{\Sigma}(2)$  & Cor.~\ref{cor:brSidesc}   \\
$\td{\Sigma}(2)$ & Sec.~\ref{sec:subhopf}  \\
$\si(2)$ &  \eqref{eq:sidef} \\
$\sibr(2)$   & \eqref{eq:sibrdef}  \\
$\sitd(2)$   & Def.~\ref{defn:S2tilde} \& Th.~\ref{thm:goodcomplex}\\
\hline
\end{tabular}
\end{center}
\caption{List of Hopf algebras and where to find them.}
\end{figure}



